DPXPlain: Privately Explaining Aggregate Query Answers

Differential privacy (DP) is the state-of-the-art and rigorous notion of privacy for answering aggregate database queries while preserving the privacy of sensitive information in the data. In today's era of data analysis, however, it poses new challenges for users to understand the trends and anomalies observed in the query results: Is the unexpected answer due to the data itself, or is it due to the extra noise that must be added to preserve DP? In the second case, even the observation made by the users on query results may be wrong. In the first case, can we still mine interesting explanations from the sensitive data while protecting its privacy? To address these challenges, we present a three-phase framework DPXPlain, which is the first system to the best of our knowledge for explaining group-by aggregate query answers with DP. In its three phases, DPXPlain (a) answers a group-by aggregate query with DP, (b) allows users to compare aggregate values of two groups and with high probability assesses whether this comparison holds or is flipped by the DP noise, and (c) eventually provides an explanation table containing the approximately `top-k' explanation predicates along with their relative influences and ranks in the form of confidence intervals, while guaranteeing DP in all steps. We perform an extensive experimental analysis of DPXPlain with multiple use-cases on real and synthetic data showing that DPXPlain efficiently provides insightful explanations with good accuracy and utility.

==> explain_linear.tex <==
\section{Explain User Question}
\label{sec:explain_linear}

\yuchao{Assume user question is a weighted sum .}

Now we consider a basic case such that the target query is a linear query as returning the difference between two counts. It captures scenarios such as asking questions about "Why the number of males is more than the number of females?", "Why the population in area A is more than the one in area B?" and "Why the number of orders in December is more than the on in October?".

Suppose we have a single dataset of $n$ tuples with $m$ categorical attributes $A_1, A_2, \ldots, A_m$, where each has domain size $d_i = d$. Suppose we are given a simple target query $E(D) = q_1(D) - q_2(D)$, where $q_1$ and $q_2$ are both counting queries. Suppose a user asks a question as $(E, high)$. Consider an impact function $I(p) = (E(D) - E(\neg p(D)))(1 - |p(D)|/|D|)$ in this case. Since $E(D)$ is linear, we can also rewrite $I(p)$ as $E(p(D))(1 - |p(D)|/|D|)$. Consider a predicate space $\mathcal{P}$ as all the possible equality predicates, which is of size $N = \prod_{i=1}^{m}(d_i+1)$. The problem is to release the top-k predicate ranked by impacts under differential privacy.

\begin{example}
Consider a dataset with $10$ binary attributes. Let $q_1$ to be the number of tuples that the first attribute is true, and $q_2$ to be the number of tuples that the first attribute is false. Suppose the user's question is about "Why $q_1$ is larger than $q_2$", which corresponds to a question $(E=q_1 - q_2, dir=high)$. Recall that in this case, the impact function $I(p; D)$ is given as $E(p(D))(1 - |p(D)|/|D|)$, where $p$ is a predicate from the all-equality predicate class $\mathcal{P}$. If these exists a predicate $p \in \mathcal{P}$ such that $E(p(D)) = 0$, which means the tuples that satisfies this predicate is divided equally by the first attribute, then its impact is 0. The goal is to find the top-10 predicates ordered by their impacts from all the equality predicates under differential privacy. In this case, the size of the all-equality predicates $\mathcal{P}$ is $3^{10} = 59049$.
\end{example}




\eat{
\begin{example}
Consider a table with 5 attributes: male or female, occupation, level of income, level of education. $q_1$ as asking the number of males in a database and $q_2$ as asking the number of females in a database. We assume some DP answers $o_1 = 102$ and $o_2 = 91$ are given, and thus $E(q_1, q_2) = o_1 - o_2 = 11$  
\end{example}
}





==> explain_non_linear.tex <==
\section{Explain a non-linear question}
\label{sec:explain_nonlinear}

The previous section focus on explaining the questions that are linear combinations of linear queries. In this section, we discuss the case that the question is an arithmetic expression of linear queries. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/explain-subsample.PNG}
        \caption{Subsample and Rank Aggregation}
        \label{fig:subsample}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/explain-subsample-rank_bound.PNG}
        \caption{Rank Bound (Rank Aggregation)}
        \label{fig:rank_bound_aggregation}
    \end{subfigure}
    \label{fig:rank_aggregation_and_bound}
\end{figure}

We first randomly partition the data into $N$ partitions. Within each partition, we find the complete rankings of all the predicates. Now consider the rank aggregation. To make it DP, we can apply existing differentially private rank aggregation to release the top-k rankings.

To bound the rank of each released predicate, we consider a conception as follows: Each partition is a voting group, and we want to say "With probability $\geq 95\%$, there are more than $95\%$ of the voting groups that vote the predicate $p$ to be within rank $j$."

\subsection{Bound by SVT}












==> framework.tex <==
\section{Framework of \oursys}

\sudeepa{See if should be merged with the intro}
%\amir{This can be part of the intro}
Our framework aims to provide an end-to-end solution for query evaluation and question explanation while data is protected under differential privacy. Data curator can set up a total privacy budget to enforce that the privacy loss can never go beyond the budget, and specify the portion of privacy budget used for each release to the user from the framework. The system is composed of three phases as \cref{fig:framework} shows. 

\textbf{Phase 1 - Submit Query \& Receive Noisy Answers.} 
In the first phase, user submits a group-by query: \emph{``\texttt{SELECT $\Agb$, agg($\Aagg$) FROM R WHERE $\phi$ GROUP BY $\Agb$}''}. Here the aggregation "agg" could be either sum, count or average. The predicate $\phi$ can be any predicate without sub-queries. Our framework will return a list of tuples $(\alpha_i, \hat{o}_i)$ for each group $\alpha_i$ from the domain of the group-by attribute $\Agb$. All the aggregation value $\hat{o}_i$ are computed in a differentially private way with privacy budget $\rhoQuery$. 

\textbf{Phase 2 - Submit Question \& Receive Noise Quantification.} 
In the second phase, user might be curious about the relationship between the group aggregations and seek for an explanation. Our framework supports two types of explanation: noise quantification and top-k explanations, depending on the question. 

In our framework, we support users to submit questions like "Why the aggregation value $\hat{o}_i$ from group $\alpha_i$ is larger than the aggregation value $\hat{o}_j$ from group $\alpha_j$?", or simply $Q = (\alpha_i, >, \alpha_j)$. Unlike standard explanation frameworks [?], 
due the added noise, although we observe $\hat{o}_i > \hat{o}_j$ from the framework releases, it is possible that the truth is $o_i \leq o_j$, the true aggregation values from two groups are in the opposite order. To remove the effect of noise in the question, we quantify the noise existing in the question as reporting a confidence interval for $o_i - o_j$ at confidence level $\gamma$ with privacy budget $\rhoQuest$. 
%If the confidence interval is above 0, with confidence $\gamma$ we can conclude that $o_i > o_j$ is true. 
%This phase costs zero privacy budget.
If 0 is included in the confidence interval, or the interval is totally below 0, we can conclude that noise is the explanation for the question since it reverses the direction from the ground truth with high probability. Otherwise, we continue and try exploring the explanations from the data.

\textbf{Phase 3 - Continue Question \& Receive Explanation.}
% In the third phase, depending on the noise quantified from the previous phase, user can choose to 
% 1) continue the question if noise does not affect the validity of the question or 2) change the question in the opposite direction if the true difference between two groups is highly likely in the opposite direction or 3) withdraw the question if user thinks that noise can sufficiently explain the question. 

In the third phase, depending on the noise quantified from the previous phase, user can choose to 
1) continue the question if noise does not affect the validity of the question or 2) stop the question if user thinks that noise can sufficiently explain the question. 

In the first case, our framework constructs an table of top-k explanations to the user. Each row consists an explanation predicate, its influence confidence interval and its rank confidence interval. An explanation predicate is a predicate with conjunctions of one or multiple clauses in the form $A = c$, where $A$ is an attribute and $c$ is a constant. We consider explanation predicate as the basic element as a factor that affects the group difference from the question, and its influence is measured by how much it can change the group difference if we remove the tuples from the database that match the explanation predicate. We also consider a set of explanation predicate $\mathcal{P}$ to select from, and rank the explanation predicates by their influences. We select top-k explanation predicates with privacy budget $\rhoTopk$, report their influence confidence interval with privacy budget $\rhoInflu$, and report their rank confidence interval with privacy budget $\rhoRank$.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/explain-framework.jpg}
    \caption{The framework of a differentially private explanation system. }
    \label{fig:framework}
\end{figure}

% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{|p{2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|}
%         \hline\multirow{2}{2cm}{Predicate $p_{r_i}$} & \multicolumn{2}{p{2.4cm}|}{95 confidence interval of $\imp(p_{r_i})$}  
%         &  \multicolumn{2}{p{2.4cm}|}{95 confidence interval of $\rank(p_{r_i})$}   \\ \cline{2-3} \cline{4-5}
%          ~ & L & R & L & R \\ \hline \hline
%           $A_1 = 1, A_2 = 1$ & 990 & 1010 & 1 & 3  \\ \hline
%           $A_1 = 1$ & 980 & 990 & 2 & 3  \\ \hline
%           $A_2 = 1$ & 90 & 110 & 3 & 5 \\ \hline
%     \end{tabular}
%     \caption{Private explanation table. $r_i$ is the predicate index of the $i$-th predicate $p_{r_i}$ selected by the private selection mechanism. $\imp$ is the impact function. }
%     \label{tbl:explanation_table}
% \end{table}





==> introduction.tex <==
\section{Introduction}
\amir{Needs some editing and emphasize the contributions after we're done with the other sections}
Differential privacy has been becoming the gold standard of the privacy protection technique. It has been applied to databases for differentially private SQL query answering. On the other hand, differential privacy is not yet applied to query explanations. In this paper, we explored this problem and proposed a framework. 

\sudeepa{edited from here ..........}

Here is an example database that we will use to illustrate our framework.

%\subsection{Demo}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{"./figures/intro_example_data_adult.png"}
%     \caption{Example of the \dataset{Adult} dataset.}
%     \label{fig:intro_example_data_adult}
% \end{figure}

\begin{figure}[t]
    \scriptsize
    \centering
    \begin{tabular}{|r|r|r|r|r|}
        \hline
        \rowcolor{gray!40}
        \textbf{marital-status} & \textbf{occupation} & $\ldots$ & \textbf{education} & \textbf{high-income} \\
        \hline
        Never-married & Machine-op-inspct & $\ldots$ & 11th & 0 \\ %\hline
        Married-civ-spouse & Farming-fishing & $\ldots$ & HS-grad & 0 \\ %\hline
        Married-civ-spouse & Protective-serv & $\ldots$ & Assoc-acdm & 1 \\ %\hline
        Married-civ-spouse & Machine-op-inspct & $\ldots$ & Some-college & 1 \\
        %\hline
        $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\ \hline
    \end{tabular}
    \caption{Example of the \dataset{Adult} dataset.}
    \label{fig:intro_example_data_adult}
\end{figure}

\begin{example}\label{ex:intro1}
Consider the \dataset{Adult} (a subset of census) dataset \cite{?} with 48,842 tuples.
We consider the following attributes:
{\tt age,}
{\tt workclass,}
{\tt 
education,}
{\tt 
marital-status,}
{\tt 
occupation,}
{\tt 
relationship,}
{\tt 
race,}
{\tt 
sex,}
{\tt 
native-country,}
{\tt 
and high-income},
where {\tt high-income} is a binary attribute indicating whether the income of a person is above 50K or not (changed to 1/0 from {\tt true/false} for easy aggregation);  some relevant columns are illustrated in \Cref{fig:intro_example_data_adult}. % by preprocessing the dataset. 
%The entire framework includes three phases: (I) the user submits a group-by aggregation query, to user submitting a question to the query result, and finally to user receiving an \exptab\ for the question. %\sudeepa{are we using explanation table? may be use a macro}.  
%\sudeepa{These are not three phases, so commenting it out}
\end{example}

Below we demonstrate the framework by a concrete query and user question using \Cref{ex:intro1}.
In the {\bf first phase (Phase-1)}, user submits a query and gets the results as shown in Figure~\ref{fig:phase1}.
This query is asking the fraction of people with high income in each marital-status group. As \Cref{fig:phase1} shows, the framework returns the answer with two columns, ``group" and ``\privans". 
Here ``group'' corresponds to the group-by attribute  {\tt marital-status}. However, since the data is private, instead of seeing the actual aggregate values avg-high-income, the user sees a perturbed answer \privans\ for each group as output by some differentially private mechanism with a given privacy budget (here computed by the Gaussian mechanism with privacy budget $\rho = 0.1$ \cite{bun2016concentrated}). 
The third column ``\trueans'' shown in \Cref{fig:phase1} corresponds to the {\bf true aggregated output} for each group; it is hidden from the user and is shown here only for illustration. 

%In the second column, all these numbers have been perturbed from the ground truth before released by some differentially private mechanisms with privacy budget $0.1$. %\red{SR:explain} 
%The third column is hidden from the user, but we show it here for illustration. 

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.3\linewidth]{"./figures/intro_example_groups_adult.png"}
%     \caption{Answer of the query.}
%     \label{fig:intro_example_groups_adult}
% \end{figure}

    \cut{
    \begin{subfigure}[b]{0.28\linewidth}
        \centering
        ``\texttt{SELECT marital-status, AVG(high\_income) FROM R GROUP BY marital-status}''
        \caption{Query}
        \label{fig:demo_query}
    \end{subfigure}
    
    
    }
%    \begin{subfigure}[b]{0.7\linewidth}
 %       \centering


\begin{figure}[h]
    \centering        
\begin{tcolorbox}[colback=white,left=1.5pt,right=1.5pt,top=0pt,bottom=0pt]
{\small 
%\begin{verbatim}
{\bf Question-Phase-1:}\\
SELECT marital-status, AVG(high-income) as avg-high-income\\
FROM R\\
GROUP BY marital-status\\

{\bf Answer-Phase-1:}
%\end{verbatim}
\begin{center}
    \newcommand{\EFFORT}[1]{\cellcolor{black!#1}}
\begin{tabular}{r|c | c} %>{\color{gray!40}}r}

    %\toprule
    \hline
    \textbf{group} & \textbf{\privans} & \EFFORT{25}\textbf{\trueans}  \\
    marital-status & avg-high-income & \EFFORT{25}(hidden) \\ \hline
    %\midrule
          Never-married  & 0.045511 & \EFFORT{25} 0.045480 \\
              Separated  & 0.064712 & \EFFORT{25}0.064706 \\
                Widowed  & 0.082854 & \EFFORT{25}0.084321 \\
  Married-spouse-absent  & 0.089988 & \EFFORT{25}0.092357 \\
               Divorced  & 0.101578 & \EFFORT{25}0.101161 \\
      Married-AF-spouse  & 0.463193 & \EFFORT{25}0.378378 \\
     Married-civ-spouse  & 0.446021 & \EFFORT{25}0.446133 \\
     \bottomrule
\end{tabular}

\end{center}
    

        %\includegraphics[width=\linewidth]{figures/intro-answer-martial.jpg}
 }       
        \end{tcolorbox}
%        \caption{Query Answer}
%        \label{fig:demo_answer}
%    \end{subfigure}
    \caption{Phase-1 of \oursys: Run a query and receive noisy answers by DP. \trueans s are not visible to the user.}
    \label{fig:phase1}
%    \label{fig:demo_query_and_answer}
\end{figure}

In the \textbf{second phase  (Phase-2)}, user selects two groups to compare their aggregate values and asks for explanations. However, unlike standard explanation frameworks \cite{?} where the answers of a query are correct and hence the question asked by the user is also correct, in the private setting, the answers that the users see are perturbed. Therefore, the user question and the direction of comparison may not be valid. Hence, instead of getting an explanation to their question, the users get an error bound on the validity of difference. Below we illustrate two such comparisons:

% ``\texttt{Why AVG(high\_income) WHERE `education` == "Prof-school" >= AVG(high\_income) WHERE `education` == "Doctorate"?}''
\begin{figure}[h]
\begin{tcolorbox}[colback=white,left=1.5pt,right=1.5pt,top=0pt,bottom=0pt]
%\begin{verbatim}
%\begin{center}
 %   {\bf (Comparison-A)}
%\end{center} 
{\bf Question-Phase-2:}\\
{Why avg-high-income of group {\tt \bf Married-AF-spouse} $>$  that of group {\tt \bf Married-civ-spouse}?}\\

{\bf Answer-Phase-2:}\\
Due to the noise injected, the actual aggregate difference for groups {\tt Married-AF-spouse} and {\tt Married-civ-spouse} might be different from what we observe from the noisy answers: $0.017$. To quantify the noise, we provide a 95\% confidence interval for group difference as $(-0.259, 0.460)$.
\end{tcolorbox}
\caption{Phase-2 of \oursys\ (Comparison-A)}
\label{fig:phase2-A}
\end{figure}

From the hidden \trueans\ column in \Cref{fig:phase1}, the group {\tt Married-AF-spouse} actually has smaller avg-high-income than the group  {\tt Married-civ-spouse}, which is totally the opposite from the question. Since the interval shown above on the noise bounds as the answer in this phase includes numbers on the negative axis, the user can conclude that the added noise might have possibly changed the direction of comparison from the ground truth. {\bf Since the validity of the user question is uncertain, we know that any further explanation might not be meaningful and the framework stops here.} In other words, the explanation of the comparison is primarily attributed to the added noise by the DP mechanism. 
\par
Now we consider the comparison between other two points:

%To quantify the noise, the framework then reports the confidence interval about the difference between two groups as \Cref{fig:demo_question_ci_1} shows. 

\begin{figure}[h]
\begin{tcolorbox}[colback=white,left=1.5pt,right=1.5pt,top=0pt,bottom=0pt]
%\begin{verbatim}
%\begin{center}
 %   {\bf (Comparison-B)}
%\end{center} 
{\bf Question-Phase-2:}\\
{Why avg-high-income of group {\bf Married-civ-spouse} $>$ that of group {\bf Never-married}?}\\

{\bf Answer-Phase-2:}\\
Due to the noise injected, the actual aggregate difference for groups {\tt Married-civ-spouse} and {\tt Never-married} might be different from what we observe from the noisy answers: $0.401$. To quantify the noise, we provide a 95\% confidence interval for group difference as $(0.399, 0.402)$.
\end{tcolorbox}
\caption{Phase-2 of \oursys\ (Comparison-B)}
\label{fig:phase2-B}
\end{figure}

%as \Cref{fig:demo_question_1} shows. 


% \cut{
% \begin{tcolorbox}[colback=white,left=1.5pt,right=1.5pt,top=0pt,bottom=0pt]
% {\bf Answer-Phase-2:}\\
% The 95\% confidence interval for the aggregate difference for groups ``Married-AF-spouse'' and ``Married-civ-spouse'' is  $(-0.237, 0.483)$.
% \end{tcolorbox}
% }



% ``\texttt{The 95\% confidence interval of the difference is  $(0.010, 0.018)$}''

% ``\texttt{The 95\% confidence interval of the difference is  $(0.135, 0.137)$}''

% \cut{
% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.54\linewidth}
%         \centering
%         ``\texttt{Why AVG(high\_income) of group "Married-AF-spouse" > AVG(high\_income) of group "Married-civ-spouse"?}''
%         \caption{Question}
%         \label{fig:demo_question_1}
%     \end{subfigure}
%     \begin{subtable}[b]{0.45\linewidth}
%         \centering
%         ``\texttt{The 95\% confidence interval of the group difference is  $(-0.237, 0.483)$}''
%         \caption{Noise quantification}
%         \label{fig:demo_question_ci_1}
%     \end{subtable}
%     \caption{Phase 2 - Submit Question \& Receive Noise Quantification.}
%     \label{fig:demo_question_and_noise_quantification_1}
% \end{figure}
% }

%Suppose user submits another question and gets the following answer in Phase 2:


%``\texttt{Why AVG(high-%income) of group "Married-civ-spouse" > \\ AVG(high-income) of group "Never-married"?}''
%as \Cref{fig:demo_question_2} shows. 
In this case, the confidence interval about the difference between two groups
%, as \Cref{fig:demo_question_ci_1} shows, 
does not include zero and is tight around a positive number 0.4, which indicates that the direction between two groups as the question is asking is correct with high probability. Since the question is valid, user may continue with the next phase for Comparison-B. 

\cut{
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.54\linewidth}
        \centering
        ``\texttt{Why AVG(high\_income) of group "Married-civ-spouse" > AVG(high\_income) of group "Never-married"?}''
        \caption{Question}
        \label{fig:demo_question_2}
    \end{subfigure}
    \begin{subtable}[b]{0.45\linewidth}
        \centering
        ``\texttt{The 95\% confidence interval of the group difference is  $(0.3995, 0.4015)$}''
        \caption{Noise quantification}
        \label{fig:demo_question_ci_2}
    \end{subtable}
    \caption{Phase 2 - Submit Question \& Receive Noise Quantification.}
    \label{fig:demo_question_and_noise_quantification_2}
\end{figure}
}

In the {\bf third phase  (Phase-3)}, for Comparison-B, user wants to know more explanations about the question from the data. To achieve this again with differential privacy, our framework reports an ``{\bf \exptab}'' to the user as \Cref{fig:phase3} shows, which includes the top-5 {\em explanation predicates}. In the simplest form, explanation predicates are singleton predicates of the form ``{\tt attribute = <value>}'', while in general, our framework supports more complex predicates involving conjunction, disjunction, and comparison ($>, >=$ etc.) \red{SR: CHECK AND UPDATE}. In \Cref{fig:phase3}, top-5 explanation predicates are shown out of 103 single attribute equality predicates, according to a (noisy) differentially private scoring function that we discuss later. Once the top-5 predicates are selected, the \exptab\ also shows both their {\em relative influence} (how much they affect the difference of noisy aggregates of the groups in the question) and their {\em ranks} in the form of confidence interval (upper and lower bounds) to preserve differential privacy. The total privacy loss in this phase is $\rho = 2$ (which includes the mechanisms for privately selecting top-k explanation predicates, privately computing confidence interval of influence and privately computing confidence interval of rank). 
%It is done in a differentially private way with privacy budget 10.

From this table, we can see that {\tt occupation = Exec-managerial} is returned as the top explanation predicate that the average high-income rate in the group {\tt Married-civ-spouse} is higher than that of the group {\tt Never-married}. The 95\%-confidence interval of its rank is narrowed down to [1, 4], so we know this is highly likely to be among the true top ones. This explanation predicate can be interpreted in this way:\\
{\em If we exclude the people whose occupation is {\tt Exec-managerial}, it is less likely that {\tt Married-civ-spouse} has higher avg-high-income rate than {\tt Never-married}.}\\
In other words, managers tend to earn more if they are married than those who are single, which probably can be attributed to the intuition that married people might be older and have more seniority. 
%See \Cref{fig:expl_in_text} for another explanation in text. Similarly, we can interpret other explanation predicates in this way. 


%\end{example}
%Next, we explain more about our framework.

% The privacy parameter is 10 for query answering and 10,000 for explanation table.

% The privacy parameter is 10 for query answering and 500 for explanation table.

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{"./figures/intro_example_explanation2_adult.png"}
%     \caption{The explanation table of the question.}
%     \label{fig:intro_example_explanation_adult}
% \end{figure}



\begin{figure}[h]
    \centering
    % \begin{subfigure}[b]{\linewidth}
    %     \includegraphics[width=\linewidth]{figures/intro-expl-martial-absolute.jpg}
    %     \caption{Absolute influence}
    % \end{subfigure}
\begin{tcolorbox}[colback=white,left=1.5pt,right=1.5pt,top=0pt,bottom=0pt]
    %\begin{subfigure}[b]{\linewidth}
        % \includegraphics[width=\linewidth]{figures/intro-expl-martial-relative.jpg}
    \small
    \begin{tabular}{@{} >{\raggedright}p{3.8cm} c c c c @{}}
        \toprule
        %predicate & Inf 95-CI L & Inf 95-CI U & Rnk 95-CI L & Rnk 95-CI U \\
        \multirow{2}{*}{explanation predicate} &
        \multicolumn{2}{c}{Rel Influ 95\%-CI} &
        \multicolumn{2}{c}{Rank 95\%-CI} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        & L & U & L & U \\
        \midrule
occupation = "Exec-managerial" &  3.60\% & 9.39\% & 1 &  6 \\
       education = "Bachelors" &  3.21\% & 8.63\% & 1 &  8 \\
              age = "(40, 50]" &  2.31\% & 8.39\% & 1 &  9 \\
 occupation = "Prof-specialty" &  2.16\% & 7.73\% & 1 & 16 \\
    relationship = "Own-child" & -0.08\% & 4.02\% & 1 & 92 \\
        \bottomrule
    \end{tabular}
\end{tcolorbox}    


     %   \caption{Relative influence \yuchao{Use the noisy difference as the denominator.}}
    %\end{subfigure}
    \cut{
    \begin{subfigure}[b]{\linewidth}
        ``Around 6\% to 7\% of the gap about high income ratio between group \textit{Married-civ-spouse} and \textit{Never-married} can be explained by people whose \textit{occupation} is \textit{Exec-managerial}, which is among the 1st to 4th reasons.''
        \caption{Explanation of the first row.}
        \label{fig:expl_in_text}
    \end{subfigure}
    }
    \caption{Phase-3 of \oursys: Receive further explanations from data for question Comparison-B (\Cref{fig:phase2-B}) that passed Phase-2.}
    \label{fig:phase3}
\end{figure}

\yuchao{We could drop this para} Notice that there is a gap between the influence confidence interval between the first explanation predicate and the last one. The rank confidence interval for the last explanation predicate is also wide. This indicates only the first top-4 explanation predicates have out-standing influences to the question, and the rest only have trivial influences. \red{SR: revisit}

\begin{figure}[h]
    \centering
    \begin{tabular}{r|c}
    \toprule
    explanation predicate & Rel Influ \\
    \midrule
occupation = "Exec-managerial"  &       6.19\% \\
       education = "Bachelors"  &       6.11\% \\
              age = "(40, 50]"  &       5.59\% \\
 occupation = "Prof-specialty"  &       4.84\% \\
         education = "Masters"  &       2.81\% \\
    \bottomrule
    \end{tabular}
    \caption{True top-k explanation predicates and their relative influences. From all the 103 explanation predicates, only 13 have relative influences larger than 1\%.}
    \label{fig:true-top-k}
\end{figure}

\sudeepa{Need to compare with other explanation work}

\textbf{Our contributions.~~}







==> other_variants.tex <==
\section{Related Work}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/explain-variants.PNG}
    \caption{The variants of the explanation framework components.}
    \label{fig:variants}
\end{figure*}

\subsection{From mechanism to sensitivity}
A DP mechanism that is related to a function $f$ could be more complicated than adding a noise scaled to the global sensitivity of the function $f$. Although we know how to evaluate the function $f$ in a DP manner using the associated DP mechanism, we cannot find the function that gives the highest value among a lot of such functions. A classical private selection mechanism requires the global sensitivity of each function is bounded. Here we provide a way to convert a DP mechanism into a global sensitivity-bounded score function:
\begin{align*}
    u(p, D) = \frac{1}{\epsilon_0} \ln\left(Pr[\mathcal{M}_p(D) \geq t]\right)
\end{align*}
, where t is a pre-defined threshold and $\epsilon_0$ is the privacy budget used for the mechanism $\mathcal{M}_p(D)$. The global sensitivity of $u(p, D)$ is 1. Since it may not be practical to find the formula of $Pr[\mathcal{M}_p(D) \geq t]$, one can use Monte-Carlo to estimate this number. 

\subsection{Large Margin Mechanism}
If the score function follows some $(\ell, \gamma)$-margin condition, i.e the difference between the top score and the $\ell+1$ largest score is larger than $\gamma$, we can apply the large margin mechanism \cite{chaudhuri2014large} to release the top-1 predicate so that the released predicate has its score not $\gamma$ smaller then the best one has probability more than 1/2. 

\subsection{Inverse Sensitivity}
Consider a score function: $u(p, D) = - min_{t}$ $\{$changing $t$ tuples in $D$ can make $p$ the top-1 predicate$\}$, and apply the exponential mechanism to find the top-1 predicate. It is shown in \cite{asi2020instance} that such a score function gives an instance-optimal utility. 

Even for a simple impact function such as $I(p) = E(p(D)) - E(D)$, it is not trivial to find the minimum of change to push a predicate $p$ to be the one of the most impact.

\subsection{Sample and Aggregate}
Given a database $D$, randomly partition it into $\ell$ disjoint subsets. For each partition, randomly re-scale it back to the size of the original database, and apply the impact function on this re-scaled database to find the top-1 predicate. Using the votes from $\ell$ partitions, we release the predicate with the highest votes as the final top-1 predicate.

The final step from the previous approach does not follow differential privacy. To turn this step into being differential private, there are multiple choices. One choice is to apply exponential mechanism where the score function is defined as the number of votes. The sensitivity for this score function is 1 because changing one user can only change the vote from one partition. 

Due to the random partition and random re-scaling, even without differential privacy, there could exist bias in this approach. However, this approach works for any complicated impact function.

\subsection{Bag of Little Bootstraps}
This approach is similar to "sample and aggregate", except that it repeats multiple random re-scaling within a partition and apply the impact function for each repetition to find the top-1 predicate. We make a vote for the most frequent top-1 predicate for each partition.

This approach was designed to find the distribution of a specific estimator. Here the estimator is the top-1 predicate. 

It is not clear whether repeating the re-scaling step can make the algorithm more robust.



\subsection{Frequent Itemsets Mining}

I don't see a clear connection to the frequent itemsets mining problem, although there is DP literature about solving this problem.

==> query.tex <==
\section{Private Release of Query Results}
% \amir{This should be somewhere else. Maybe a small section about the evaluation?}
% \yuchao{Put it into a file and put after the model section temporarily, call it phase-1, but not part of the problems because it it not novel but still the part of the framework. At each sec, say what phase it is into and what problem it is about. }
\yuchao{Make it shorter and put it into the background.}

In this section, we discuss Phase 1, the private release of query results. It is not related to any problem defined in \cref{sec:problem_defs}, but for the completeness of the framework we elaborate the details as follows. 

A group-by aggregation query \texttt{SELECT $\Agb$, agg($\Aagg$) FROM R WHERE $\phi$ GROUP BY $\Agb$} returns a list of tuples $(\alpha_i, o_i)$ where $\alpha_i \in \dom(\Agb)$. Since no single tuple can exist in more than one group, adding or removing a single tuple can at most change the result of a single group. Formally, according to the parallel composition rule \cite{bun2016concentrated}, if we can release $o_i$ under $\rho$-zCDP for each $\alpha_i \in \dom(\Agb)$, the entire release satisfies $\rho$-zCDP.

For a $CNT$ or $SUM$ query, we can use Gaussian mechanism as adding Gaussian noise $N(0, \sigma^2)$ to the query result $o_i$ for each group $\alpha_i$: $\hat{o}_i = o_i + N(0, \sigma^2)$, where the noise scale $\sigma$ is proportional to the query sensitivity $\Delta_q$: $\sigma = \frac{\Delta_q}{\sqrt{2\rho}}$ to satisfy $\rho$-zCDP. For a $CNT$ query, the sensitivity $\Delta_q$ is 1. For a $SUM$ query, the sensitivity $\Delta_q$ is $\dommax{\Aagg}$, the maximum absolute value of the aggregation attribute in its domain. 

For an $AVG$ query, each group result $o_i$ can be decomposed by a $SUM$ query and a $CNT$ query as a division between them. We denote by $q^{SUM}_i(D) = SUM(\Aagg, (\phi \land \Agb=\alpha_i)(D))$ as the sum of group $\alpha_i$ and $q^{CNT}_i(D) = CNT(\Aagg, (\phi \land \Agb=\alpha_i)(D))$ as the count of group $\alpha_i$. Therefore, $o_i = q^{SUM}_i(D) / q^{CNT}_i(D)$ as a division between a $SUM$ query and a $CNT$ query. 
We then divide privacy budget $\rho$ into halves, use Gaussian mechanism for each query just as the previous CNT or SUM case, and finally take the division between two noisy results as the final release $\hat{o}_i = \hat{o}^{SUM}_i / \hat{o}^{CNT}_i$, where  $\hat{o}^{SUM}_i = q^{SUM}_i(D) + N(0, \sigma_{SUM}^2)$,  $\hat{o}^{CNT}_i = q^{CNT}_i(D) + N(0, \sigma_{CNT}^2)$,  $\sigma_{SUM} = \frac{\dommax{\Aagg}}{\sqrt{2\rho/2}}$ and $\sigma_{CNT} = \frac{1}{\sqrt{2\rho/2}}$. It satisfies $\rho$-zCDP by the composition rules \cite{bun2016concentrated} since each satisfies $\rho/2$-zCDP and the total privacy loss is the sum of each privacy loss. 

Another way to privately answer an AVG query is to apply Gaussian mechanism directly to the query answer, but as \cref{tbl:user_query_sensitivity} shows, the sensitivity of $AVG$ is as large as the range of the query itself, which results in higher error. User query answering is the phase 1 of this framework.

\begin{table}[htp!]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{type} & $CNT$ & $SUM$ & $AVG$   \\
        \hline 
        \textbf{sensitivity} & $1$ & $\dommax{\Aagg}$ & $\dommax{\Aagg}$ \\ \hline
    \end{tabular}
    \caption{Sensitivity of a user query}
    \label{tbl:user_query_sensitivity}
\end{table}

==> rank_ci.tex <==
\subsection{Confidence Interval of Predicate Rank}\label{sec:private_rank_ci}

Our goal in this section is to find the confidence interval of the explanation predicate rank to solve Problem \ref{pro:private_rank_ci}. In the third phase of this framework (Figure \ref{fig:framework}), after we have selected the noisy top-k explanation predicates (Section \ref{sec:private_topk}) and found the confidence intervals of their influences (Section \ref{sec:private_influence_ci}), we derive confidence intervals of the rank for each explanation predicate with a total privacy budget of $\rhoRank$.
The idea behind our approach is find the lower and upper bound of the interval using random binary search, where the randomness stems from the random noise added to the private score during the search.

% We start with a naive approach and explain why it does not work, and then introduce our noisy binary search algorithm that tackles this challenge.

% \subsection{Random Binary Search}

% Instead, we introduce a binary search algorithm to find the bounds of the confidence interval of rank. It works by sorting all the explanation predicates by the score function discussed in \cref{sec:private_topk}, which has low sensitivity and also keeps the order of predicates as sorted by influences, and use binary search to find the rank of which the corresponding score is close to the score of the target explanation predicate. 
%The score function for a typical influence function is defined in the same way as \cref{tab:scoring_function}. 

% Since adding or removing an tuple could possibly change the ranks of a non-trivial amount of predicates, the rank of any explanation predicate has a high sensitivity and thus it is not feasible to directly add a noise to the rank and infer an confidence rank bound.
% However, 

Given an explanation predicate $p$, our framework aims to privately report a confidence interval of its rank from a set of explanation predicates $\mathcal{P}$ sorted by the influence function $\imp$, or $\rank(p; D, \mathcal{P}, \imp)$. For example, $\I_{rank} = (1, |\mathcal{P}|)$ is a trivial confidence interval which has no privacy loss and always includes the true rank. 
Since $\rank(p;$ $D, \mathcal{P}, \score)$ $=$  $\rank(p; D, \mathcal{P}, \imp)$ by \Cref{pro:score_influ_order}, we focus on $\rank(p;$ $D, \mathcal{P}, \score)$ instead. 

One approach to this problem is to analyze the sensitivity of $\rank(p; D, \mathcal{P}, \score)$ and add a Gaussian noise to derive a confidence interval. However, the sensitivity of rank is high, since adding one tuple could possibly changing the highest score to be the lowest and vice versa. 

Although the sensitivity of rank is high, we find a critical observation about rank and score. 
\begin{observation}
The score at a fixed rank has low sensitivity. 
\end{observation}
Take the score at rank 1 as an example. Given two neighboring datasets, even if the top-1 explanation predicates are different from two datasets, their scores are close. Indeed, the sensitivity of the score at a fixed rank is the same as the sensitivity of the score itself. That means, given two neighboring datasets, if we sort the scores of explanation predicates in each case, align these scores from the first to the last, the difference of each pair of scores will be bounded and cannot be larger than the sensitivity of the score function. To illustrate, we denote by $\topk(t; D, \mathcal{P}, s)$ as the explanation predicate from $\mathcal{P}$ with rank $t$ that is sorted by the score function $s$ based on database $D$, and give the following theorem.

\begin{restatable}{theorem}{rankScoreSens}
\label{thm:indicator_sens}
Given a set of predicate $\mathcal{P}$, an score function $\score$ with global sensitivity $\Delta_{\score}$ and a number $t$, $\score(\topk(t; D, \mathcal{P}, \score); D)$ has global sensitivity $\Delta_{\score}$.
\end{restatable}

The intuition behind this theorem is that, fixing an explanation predicate $p$, for a neighboring dataset, if its score is increased, its rank will be moved to the top and push down other explanation predicates with lower scores, so the score at the original rank of $p$ in the neighboring dataset is still low. 

Given this observation, we develop an intelligent guessing strategy to find the rank of the target explanation predicate. Each time we make a guess about the target rank, use Gaussian mechanism to get a noisy estimate of the difference between the score of the target explanation predicate and the score at that rank . If this difference is close to 0, it indicates that this guess is highly likely to be the correct guess. Since each guess will cost some privacy budget, we use an efficient strategy, binary search, to minimize the rounds of guess to be the logarithm of the size of the explanation predicates. Due to the noise, we cannot find the target rank precisely. Instead, we first find a rank upper bound, a rank such that the true rank of the target explanation predicate is smaller than this rank with high probability, and similarly find a rank lower bound. Together, we merge two bounds into a confidence interval.


\Cref{alg:find_rank_ci} summarizes this approach.  It takes as input a list of explanation predicates and output confidence intervals of ranks for each.
We start from introducing the sub-routine \textsc{RankBound}, and then explaining how we use it for the final confidence interval. In \cref{lin:cirank_rankbound}, \textsc{RankBound} takes three parameters: an explanation predicate $p$, a privacy budget $\rho$, a sub confidence level $\beta$ and a direction $dir \in \{lower, upper\}$. It guarantees that it will find a lower or upper bound of rank with confidence $\beta$ for the explanation predicate $p$ using privacy budget $\rho$. 
In \cref{lin:cirank_depth}, we set the maximum depth $N$ of the binary search.
In \cref{lin:cirank_noise_scale}, we set the noise scale $\sigma$. It depends on the sensitivity of $s(p; D) - s(\topk(t; D, \mathcal{P}, s); D)$, which is $2\Delta_s$; and the number of Gaussian mechanisms used in the binary search, which is $N$. 
In \cref{lin:cirank_bs_init}, we initialize the binary search by setting two pointers, $t_{low}$ and $t_{high}$, as the first and last rank. 
In line \ref{lin:cirank_bias} and \ref{lin:cirank_set_margin}, we set the margin width $\xi$ and the margin according to the direction. The purpose of margin will be explained later.
Between line \ref{lin:cirank_bs_start} and \ref{lin:cirank_bs_end} is the while loop of the binary search. In \cref{lin:cirank_bs_middle}, we pick a rank that is at the middle of two pointers. In \cref{lin:cirank_indicator}, we compute the true score difference, the gap between the score of the target explanation predicate and the score of the explanation predicate that has rank $t$, and in \cref{lin:cirank_noisy_indicator} we get a noisy score difference by adding Gaussian noise with scale $\sigma$. From line \ref{lin:cirank_compare_start} to \ref{lin:cirank_compare_end} we update one of the pointer according to the noisy score difference and the margin. If we are trying to find an rank upper bound with high probability, we want the binary search to find the rank such that its score is smaller than the score of the target explanation predicate. This requires the true score difference to be non-negative. Due to the noise injected, even if noisy score difference is non-negative, the true score difference could be negative. To ensure the true score difference is non-negative with high probability, we requires the noisy score difference to be larger than a margin, which is reflected by \cref{lin:cirank_compare_start}. Then in line \ref{lin:cirank_move_high} and \ref{lin:cirank_move_low}, we move the pointer according to the comparison of the noisy score difference and the margin. The strategy is similar when we are looking for a rank lower bound, which is the case when $dir = lower$.

Next, we detail the usage of sub-routine \textsc{RankBound} to find a confidence interval. 
In \cref{lin:cirank_rho}, we divide the privacy budget $\rhoRank$ by the number of explanation predicates of which we need to find confidence intervals of rank.
In \cref{lin:cirank_beta}, we set the sub confidence level as $\beta = (\gamma+1)/2$, so that the final confidence interval has confidence level $2 \beta - 1 = \gamma$.
In lines \ref{lin:cirank_l} and \ref{lin:cirank_r}, we divide privacy budget $\rho$ by the split factor $\mu$, which is by default $0.9$, and make two calls to the sub-routine \textsc{RankBound} to find a rank upper bound and a rank lower bound for the explanation predicate $p_{r_u}$, and finally at \cref{lin:cirank_ci} merge them into a single confidence interval. We repeat this for each explanation predicate.

%\yuchao{Check the case when there exists tie}

\begin{algorithm}
\caption{Compute Confidence Interval of Rank}
\begin{algorithmic}[1]
\Require A dataset $D$, a predicate space $\mathcal{P}$, a score function $s$ with sensitivity $\Delta_s$, explanation predicates $p_{r_1}, p_{r_2}, \ldots, p_{r_k}$, a confidence level $\gamma$, a privacy parameter $\rhoRank$ and a split factor $\mu \in (0, 1)$.
\Ensure A list of $\gamma$-level confidence intervals of the influence $\rank(p_{r_u}; D, \mathcal{P}, \imp)$ for $u \in \{1, 2, \ldots, k\}$.
\Function{RankBound}{$p, \rho, \beta, dir$}
\label{lin:cirank_rankbound}
\State $N \gets \lceil\log_2\abs{\mathcal{P}}\rceil$
\label{lin:cirank_depth}
\State $\sigma \gets (2 \Delta_s) / \sqrt{2(\rho/N)}$
\label{lin:cirank_noise_scale}
\State $\xi \gets \sigma\sqrt{2\ln(N / (1-\beta))}$
\label{lin:cirank_bias} 
\State $t_{low}, t_{high} \gets 1, \abs{\mathcal{P}}$
\label{lin:cirank_bs_init}
\State 
\vspace{-10pt}
\begin{align*}
    \hspace{-70pt}
    margin \gets \begin{cases}
        \xi &, dir = upper \\
        -\xi &, dir = lower
    \end{cases}
\end{align*}
\vspace{-10pt}
\label{lin:cirank_set_margin}
\While{$t_{high} > t_{low}$}
\label{lin:cirank_bs_start}
    \State $t \gets \lfloor\frac{t_{high} + t_{low}}{2}\rfloor$
    \label{lin:cirank_bs_middle}
    \State $S \gets s(p; D) - s(\topk(t; D, \mathcal{P}, s); D)$
    \label{lin:cirank_indicator}
    \State $\hat{S} \gets S + \mathcal{N}(0, \sigma^2)$
    \label{lin:cirank_noisy_indicator}
    \If {$\hat{S} \geq margin $ }
    \label{lin:cirank_compare_start}
        \State $t_{high} \gets \max\{t-1, 1\}$
        \label{lin:cirank_move_high}
    \Else
        \State $t_{low} \gets \min \{t+1, \abs{\mathcal{P}}\}$
        \label{lin:cirank_move_low}
    \EndIf
    \label{lin:cirank_compare_end}
\EndWhile
\label{lin:cirank_bs_end}
\State \Return $t_{high}$
\label{lin:cirank_return_bound}
\EndFunction
\label{lin:cirank_rankbound_end}
\For{$u \gets 1, 2, \ldots, k$}
    \label{lin:cirank_for_start}
    \State $\rho \gets \rhoRank / k$
    \label{lin:cirank_rho}
    \State $\beta \gets (\gamma+1)/2$
    \label{lin:cirank_beta}
    \State $\I^L_u \gets \Call{RankBound}{p_{r_u}, (1-\mu)\rho, \beta, lower}$
    \label{lin:cirank_l} 
    \State $\I^U_u \gets \Call{RankBound}{p_{r_u}, \mu\rho, \beta, upper}$
    \label{lin:cirank_r} 
    \State $\I_{u} \gets (\I^L_u, \I^U_u)$
    \label{lin:cirank_ci} 
\EndFor
\label{lin:cirank_for_end}
\State \Return $\I_1, \I_2, \ldots, \I_k$
\end{algorithmic}
\label{alg:find_rank_ci}
\end{algorithm}


We now show that \Cref{alg:find_rank_ci} satisfies the privacy requirement, outputs valid confidence intervals and has a closed-form utility bound. The proof of differential privacy follows the composition theorem and the property of Gaussian mechanism \cite{bun2016concentrated}. The proof of confidence interval and its utility bound is based on the property of the random binary search. We defer the formal proof to the full version.

\begin{restatable}{theorem}{rankCI}
\label{thm:rank_ci}
Given a dataset $D$, a predicate space $\mathcal{P}$, a score function $s$ with sensitivity $\Delta_s$, explanation predicates $p_{r_1}, p_{r_2}, \ldots, p_{r_k}$, a confidence level $\gamma$, a privacy parameter $\rhoRank$ and a split factor $\mu$, \Cref{alg:find_rank_ci} returns a list of confidence intervals $\I_1, \I_2, \ldots, \I_k$ such that
\begin{enumerate}[noitemsep,topsep=0pt]
    \item \Cref{alg:find_rank_ci} satisfies $\rhoRank$-zCDP.
    \item For $\forall u \in \{1, 2, \ldots, k\}$, $\I_u$ is a $\gamma$ level confidence interval of $\rank(p; D, \mathcal{P}, \imp)$.
    \item For $\forall u \in \{1, 2, \ldots, k\}$ and $\forall x \geq 0$, the confidence interval $\I_u = (\I^L_u, \I^U_u)$ satisfies
    \begin{align*}
        Pr[
            & s(\topk(\I_{rank}^R; D, \mathcal{P}, \imp); D) - (\xi + \sqrt{2(x+\ln N)})  \\
            & \leq s(p, D) \\
            & \leq s(\topk(\I_{rank}^L; D, \mathcal{P}, \imp); D) + (\xi + \sqrt{2(x+\ln N)})]  \\
        \geq & 1 - 2e^{-x}
    \end{align*}
\end{enumerate}
\end{restatable}

%Notice that $\xi$ is proportional to $\sigma$, $\sigma$ is proportional to $\sqrt{N}$, $N$ is proportional to $\log \abs{\mathcal{P}}$.



% \begin{algorithm}
% \caption{Algorithm of Confidence Rank Bound}
% \begin{algorithmic}[1]
% \Require A dataset $D$, a predicate space $\mathcal{P}$, a score function $u$ with sensitivity $\Delta_u$, a predicate $p$, a confidence level $\gamma$ and a privacy parameter $\rho$.
% \Ensure A confidence interval of rank.
% \Function{RankUpperBound}{$\sigma, \xi$}
% \State $t_{low}, t_{high} \gets 1, \abs{\mathcal{P}}$
% \While{$t_{high} > t_{low}$}
%     \State $t \gets \lceil\frac{t_{high} + t_{low}}{2}\rceil$
%     \State $S \gets u(p; D) - u(\topk(t; D, \mathcal{P}, u); D)$
%     \State $\hat{S} \gets S + \mathcal{N}(0, \sigma^2)$
%     \If {$\hat{S} > \xi$}
%         \State $t_{high} \gets \max\{t-1, 1\}$
%     \Else
%         \State $t_{low} \gets t$
%     \EndIf
% \EndWhile
% \State \Return $t_{high}$
% \EndFunction
% \Function{RankLowerBound}{$\sigma, \xi$}
% \State $t_{low}, t_{high} \gets 1, \abs{\mathcal{P}}$
% \While{$t_{high} > t_{low}$}
%     \State $t \gets \lfloor\frac{t_{high} + t_{low}}{2}\rfloor$
%     \State $S \gets u(p; D) - u(\topk(t; D, \mathcal{P}, u); D)$
%     \State $\hat{S} \gets S + \mathcal{N}(0, \sigma^2)$
%     \If {$\hat{S} < -\xi$}
%         \State $t_{low} \gets \min \{t+1, \abs{\mathcal{P}}\}$
%     \Else
%         \State $t_{high} \gets t$
%     \EndIf
% \EndWhile
% \State \Return $t_{low}$
% \EndFunction
% \State $N \gets \lceil\log_2(\abs{\mathcal{P}}+1)\rceil$
% \State $\sigma \gets (2 \Delta_I) / \sqrt{2((\rho/2)/N)}$
% \State $\beta \gets \frac{\gamma+1}{2}$ 
% \State $\xi \gets \sigma\sqrt{2\ln(N / (1-\beta))}$
% \State $\I_{rank}^L \gets \Call{RankLowerBound}{\sigma, \xi}$
% \State $\I_{rank}^U \gets \Call{RankUpperBound}{\sigma, \xi}$
% \State $\I_{rank} \gets (\I_{rank}^L, \I_{rank}^U)$
% \State \Return $\I_{rank}$
% \end{algorithmic}
% \label{alg:find_rank_ci}
% \end{algorithm}


% For example, for the upper bound, our goal is to find a rank such that the true rank is smaller than this rank with high probability. To achieve this, we can guess a rank, and test whether it is an upper bound of rank in a differential private and low false-positive way. One guess might not be sufficient to have a rank bound that is close enough to the target explanation predicate, so we can do binary search to make it close. For each iteration, we look at a position $t$ and check the indicator function, the difference between $I(p; D)$ and $I(\topk(t; D, \mathcal{P}, I); D)$, in a noisy way to decide the next branch of the binary search. Here we denote by $\topk(t; D, P, \imp)$ as the predicate with rank $t$. Notice that when $t = \rank(p; D, \mathcal{P}, I)$, the difference (without noise) becomes 0. During the check, if the noisy difference is larger than a bias term $\xi$, we move the "high" boundary to $t-1$; otherwise, we move the "low" boundary to $t$. Two boundaries will converge to be the same and algorithm then stops and reports the boundary as the rank bound. The bias term $\xi$ is chosen such that it is guaranteed to have a low false-positive rate such that the final boundary is a true rank bound. To find the lower bound of rank, we have a similar approach.




==> topk.tex <==
\section{Private Top-k explanation Predicates}
\label{sec:private_topk}

\yuchao{Merge the following three sections into one.}

In this section, our goal is to find the top-k explanation predicates from a set of explanation predicates $\mathcal{P}$ ordered by their influences to solve Problem \ref{pro:private_topk}. This is also the first step in the third phase of our framework (Figure \ref{fig:framework}). 
% which serves to provide the ranking of predicates according to their influence. 
% the clues about the possible reasons for the phenomenon described in the user question.

% To solve it under differential privacy, we use exponential mechanism (EM) \cite{dwork2014algorithmic} to privately select k explanation predicates in a random way, such that the probability of a predicate being selected is associated with its score that is determined by a score function.

To provide the ranked explanation predicates while satisfying DP, we employ a variant of the popular exponential mechanism (EM) \cite{dwork2014algorithmic}, such that it orders the explanation predicates by their scores, which keep the same ranking as by influences, and it then reorders the explanation predicates
%, such that the probability of an explanation predicate being selected is associated with its influence.
according to their noisy scores. The noisy scores will have less distortion to the ranking if the noises injected are small, which is determined by the score sensitivity.
As we will show, using influence (Definition \ref{def:impact_function}) as score provides faithful rankings when the aggregate is CNT and SUM. 
However, for AVG, we have to augment the influence function so its sensitivity will be bounded. 
We first discuss the sensitivity of our influence function for the CNT, SUM, and AVG, and then introduce the algorithm for selecting top-k explanation predicates while preserving DP.

\subsection{Augmenting the Influence Function for Ranking} 

% Given a group-by aggregation query and a user question from the second phase, we can assign an influence value to each explanation predicate $p \in \mathcal{P}$ (using Definition \ref{def:impact_function}). This gives an ordering of the predicates in $\mathcal{P}$. We want to find the ones that are ranked within top-k and report them to the user; however, this ordering is based on the original database and revealing it directly will violate differential privacy.

% Our solution relies on the EM \cite{dwork2014algorithmic}. EM considers a set of candidates, each associated with a score, and randomly select a candidate by the weight as its exponential score. It is more likely to select the candidate with the highest score if the sensitivity of the score function is low and privacy budget is high. Therefore, we focus on bounding the sensitivity of the influence function, so that the ranking given to us by the EM will be as accurate as possible.

As we will show, our solution for privately selecting top-k explanation predicates requires a score function $s: \mathcal{P} \times \mathcal{D} \rightarrow \mathcal{R}$ that maps an explanation predicate $p$ and a database $D$ to a score. The global sensitivity of the score function, $\Delta_{\score}$, over all the predicates and all the neighboring datasets is defined as $\Delta_{\score} = \max_{p \in \mathcal{P}} \max_{D \sim D'} \abs{u(p, D) - u(p, D')}$.
%, which determines which one should be selected with higher probability. 
In our setting, we want the score function to reflect the ordering of the influences, and keep the sensitivity to be low. 
% since EM tends to select the one with the highest score. 
% The sensitivity of the score function needs to be low, so EM is more likely to select the one with the highest score.
If the sensitivity of the score function is high, the noises injected to the scores will also tend to be high. This increases the possibility that the smallest score becomes the highest score and vice versa, which greatly distorts the order of explanation predicates.

Using the influence function as the score function is the most natural choice. For $CNT$ and $SUM$, although it includes a multiplication with the normalizer, we prove the sensitivity of the influence function is bounded by $6$ and $6 \dommax{\Aagg}$ (as stated below). However, for $AVG$, the sensitivity of the average query for a single group  is high by itself \cite{li2016differential}, which is shown by the example below, not to mention the sensitivity of the influence function, which involves multiple average queries and a multiplication with the normalizer. 

\begin{example}
Consider a database with a single attribute with domain as $[0, 10^{10}]$ and 9 tuples with value 0. The average in this case is 0. However, we can add a tuple with value $10^{10}$ and change the average to be $10^9$, which indicates a high sensitivity.
\end{example}

%Recall that in Example \ref{emp:high_sens_influ}, we illustrate the high sensitivity problem for the Scorpion influence function which is in the form of a ratio. The same intuition can be applied to the $AVG$ case, which is also a ratio between a sum and a count. \amir{give a concrete example here, not just intuition}

To solve the sensitivity problem for $AVG$, while also allowing the score function to keep the order of influences, we multiply the influence function by a constant, and prove that it satisfies both requirements. This constant is determined by the user question. 
% In the new score function, it does not change as the input explanation predicate changes, so it preserves the ordering of the explanation predicates by their original influences. 


\begin{definition}[Score Function]\label{def:score-func}
% \amir{Complete the formal definition}
Given a database $D$ and a user question $\userquery = (\alpha_i, >, \alpha_j)$ with respect to the query \texttt{SELECT $\Agb$, agg($\Aagg$) FROM R WHERE $\phi$ GROUP BY $\Agb$}, the influence of an explanation predicate $p$ is defined follows: \\
\begin{small}
$\score(p; Q, D) =$
\(\begin{cases}
\imp(p; Q, D),  & agg \in \{CNT, SUM\} \\
\imp(p; Q, D) \cdot (\max_{t \in \{i, j\}} \abs{g_t (D)} + 1),  & agg = AVG
\end{cases}\)
\end{small}
\end{definition}

%\amir{Use the running example to demonstrate the ranking of the predicates}

\begin{example}
\label{ex:score}
Continue with the example in the introduction. Suppose we consider a set of explanation predicates $\mathcal{P}$ as $p_1 = $, $p_2 = $, $p_3 = $, $p_4 = $, and $p_5 = $ for the second question about average high\_income. Their influences are $\ldots$, and their scores are $\ldots$. The ranking of the explanation predicates are the same both by influences and by scores. \yuchao{Add numbers}
\end{example}

\begin{proposition}
\label{pro:score_influ_order}
The function $s$ gives the same order of explanation predicates as the influence function in Definition \ref{def:impact_function}. 
\end{proposition}


% \cref{tab:scoring_function} gives a summary of the score functions for these three types and their sensitivities. 
% Below we list the theorems for the sensitivities of different score functions. Due to the space limit, we defer the proofs to the full version. 

% \begin{table}[htp!]
%     \centering
%     \begin{tabular}{@{} c p{2cm} c c @{}}
%         \toprule
%         agg & score $u(p,  D)$ & order preserving? &
%         sensitivity \\
%         \midrule
%         CNT & $\score(p; Q, D)$ & Yes (Trivial) & 6 (Thm. \ref{thm:cnt_influ_sens})  \\
%         SUM & $\score(p; Q, D)$ & Yes & $6 \dommax{\Aagg}$   \\
%         AVG & $\score(p; Q, D) \times (\max_{t \in \{i, j\}} \abs{g_t(D)} + 1)$ & Yes & $16 \dommax{\Aagg}$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Score functions for different aggregations and corresponding sensitivities. 
%     %\amir{Is there a proof that the score func for AVG preserves the ranks?}
%     }
%     \label{tab:scoring_function}
% \end{table}


%\yuchao{Add example for why the influence function of avg is high.}

The theorem below guarantees the sensitivity of the score function. We give an intuitive proof as follows. When $agg = CNT$, we combine two group differences in the influence function into a single group difference, which is considered as a subtraction between two counting queries. The sensitivity of a counting query after a multiplication with the normalizer will multiply its original sensitivity by 3. Since we have two counting queries, the final sensitivity is 6. When $agg = SUM$, the proof is similar except we need to multiply the sensitivity by $\dommax{\Aagg}$.  For $AVG$, by multiplying by a constant, intuitively, we change $AVG$ to $SUM$, and, therefore, reduce to the case of $SUM$ and bound the sensitivity. Formal proofs are deferred to the full version \cite{?} \amir{add folder link and cite}, due to space restrictions.

\begin{restatable}{theorem}{scoreSens}[Score Function Sensitivity]
\label{thm:score_sens}
Given an explanation predicate $p$ and an user question $Q$ with respect to a group-by query with aggregation $agg$, the following holds:
\begin{enumerate}
    \item If $agg = CNT$, the sensitivity of $\score(p; Q, D)$ is 4.
    \item If $agg = SUM$, the sensitivity of $\score(p; Q, D)$ is $4~\dommax{\Aagg}$.
    % i.e., $\max_{D \sim D'} \abs{\imp(p; Q_{SUM}, D) - \imp(p; Q_{SUM}, D'} \leq 6 \max\abs{A_i}$
    \item If $agg = AVG$, the sensitivity of $\score(p; Q, D)$ is $16~\dommax{\Aagg}$.
\end{enumerate}
\end{restatable}

% \begin{theorem}[Score Function Sensitivity]

% \end{theorem}



\subsection{Noisy Top-K Ranking}

% Given a score function $u$ that is defined in the previous section, 
Once we have a score function, $\score$,
EM \cite{dwork2014algorithmic} randomly samples a predicate $p$ from $\mathcal{P}$ with probability proportional to $exp(\frac{\epsilon \score(p, D)}{2 \Delta_{\score}})$ with some privacy parameter $\epsilon$. 
% \begin{align*}
    % \Delta_{\score} = \max_{p \in \mathcal{P}} \max_{D \sim D'} \abs{u(p, D) - u(p, D')} 
% \end{align*}
Let us denote this mechanism as $\mathcal{M}_E$. We first apply $\mathcal{M}_E$ to find one explanation predicate, remove it from the entire explanation predicate space, and then apply $\mathcal{M}_E$ again until k explanation predicates are found. 
%In total, this approach satisfies $k\epsilon^2/8$-zCDP \cite{DBLP:conf/alt/Cesar021} \amir{should be a small proposition}. 
It was shown by previous work \cite{DBLP:conf/nips/DurfeeR19} that this process is identical to adding i.i.d. Gumbel noise 
%with scale $\frac{2 \Delta_u}{\epsilon u(p, D)}$ 
to each score and release the top-$k$ predicates by the noisy scores. 
We, therefore, use this fact to devise an equivalent solution that is presented by Algorithm \ref{alg:noisy_topk}.
In line 1, we set the noise scale $\sigma$ as $2\Delta_s\sqrt{k/(8\rhoTopk)}$. $\rhoTopk$ is the privacy budget for \cref{pro:private_topk}. $\Delta_s$ is the sensitivity of the score function, depending on the aggregation type. In lines 2--4, we randomly sample Gumbel noise with scale $\sigma$ and add it to the score of each explanation predicate from the space $\mathcal{P}$. In line 5, we sort the noisy scores in the descending order, and in line 6, we find the top-k explanation predicates by their noisy scores.

\begin{algorithm}
\caption{Noisy Top-k Predicates}
\begin{algorithmic}[1]
\Require A private database $D$, a group-by query $q$, a user question $Q$, a score function $\score$ with sensitivity $\Delta_{\score}$, a set of explanation predicates $\mathcal{P}$, a privacy parameter $\rhoTopk$ and a size parameter $k$.
\Ensure Top-k explanation predicates.
%\State $\epsilon \gets \sqrt{8\rho/k}$
\State $\sigma \gets 2\Delta_{\score}\sqrt{k/(8\rhoTopk)}$
\For {$i \gets 1 \ldots \abs{\mathcal{P}}$}
    % \State $s_i \gets u(p_i, D) + Gumbel(2\Delta_u/\epsilon)$
    \State $s_i \gets \score(p_i; Q, D) + Gumbel(\sigma)$
\EndFor
\State Sort $s_1 \ldots s_{\abs{\mathcal{P}}}$ in the descending order.
\State Let $r_1, r_2, \ldots, r_k$ be the indices of the top-k elements in the list.
\State \Return $p_{r_1}, p_{r_2}, \ldots, p_{r_k}$
\end{algorithmic}
\label{alg:noisy_topk}
\end{algorithm}

\begin{example}
%\amir{Demonstrate the algo. using the running example}
Continue with example in the introduction. For the second question, we have in total ? predicates as the set of explanation predicates. For each of the explanation predicate, we add a Gumbel noise with scale $\sigma = ?$ to their score. For example, for the predicates in \Cref{ex:score}, their noisy scores are $\ldots$. Finally, we sort explanation predicates by their noisy scores and report the top-k. \yuchao{Add numbers} 
\end{example}

The following theorem guarantees that Algorithm \ref{alg:noisy_topk} satisfies DP and that the returned list of top-k predicates is close to that of the true top-k. The proof of differential privacy follows \cite{DBLP:conf/nips/DurfeeR19}. The proof of utility is based on the utility theorem of EM in Thm 3.11 of \cite{dwork2014algorithmic}. 

\begin{restatable}{theorem}{PrivateTopk}
\label{thm:private_top_k}
Given a private database $D$, a group-by query $q$, a user question $Q$, a score function $\score$ with sensitivity $\Delta_{\score}$, a predicate space $\mathcal{P}$, a privacy parameter $\rhoTopk$ and a size parameter $k$, the following holds:
\begin{enumerate}
    \item Algorithm \ref{alg:noisy_topk} finds k explanation predicates while satisfying $\rhoTopk$-zCDP.
    \item Denote by $OPT^{(i)}_{\score}(D)$ the $i$-th best score, and by $\mathcal{M}^{(i)}_{E}$ the $i$-th explanation predicate returned by Algorithm \ref{alg:noisy_topk}. For $\forall t$ and $\forall i \in \{1, 2, \ldots, k\}$, we have
    \begin{small}
    $$Pr\left[\score(\mathcal{M}^{(i)}_{E}; Q, D) \leq OPT^{(i)}_{\score}(D) - \frac{2\Delta_s}{\sqrt{8\rhoTopk/k}}(\ln(|\mathcal{P}|) + t)\right] \leq e^{-t}$$
    \end{small}
\end{enumerate} 
\end{restatable}

%\amir{intuition for the proof?}



% \begin{proposition}
% Denote $OPT^{(i)}_u(D)$ to be the $i$-th best score, and $\mathcal{M}^{(i)}_{E}$ to be the $i$-th explanation predicate returned from \cref{alg:noisy_topk}. For $\forall t$ and $\forall i \in \{1, 2, \ldots, k\}$, we have $$Pr\left[u(\mathcal{M}^{(i)}_{E}, D) \leq OPT^{(i)}_u(D) - \frac{2\Delta(u)}{\sqrt{8\rho/k}}(\ln(|\mathcal{P}|) + t)\right] \leq e^{-t}$$.
% \end{proposition}

% \yuchao{Remove this sec and discuss the space problem in the experiment section.}
% \paratitle{The class of explanation predicate set}
% Exponential mechanism basically assign a probability distribution over the entire set of explanation predicates $\mathcal{P}$. This implies that the space of the predicates should be finite, which means that we exclude the set of explanations predicates such as $\mathcal{P} = \{A \geq c | c \in \mathbb{R}\}$. Secondly, the choice of the set of explanation predicates cannot depend on the data, otherwise it violates differential privacy; this implies that we cannot use the active domain of the data to specify the set of explanation predicates, which means that we exclude the set of explanations predicates such as $\mathcal{P} = \{A \geq c | c \in \text{active domain of}~A~\text{in}~D\}$. \amir{What is the goal of this discussion?}









